Consistency Prototype Module and Motion Compensation for Few-Shot Action Recognition (CLIP-CP$\mathbf{M^2}$C)

Recently, few-shot action recognition has significantly progressed by learning the feature discriminability and designing suitable comparison methods. Still, there are the following restrictions. (a) Previous works are mainly based on visual mono-modal. Although some multi-modal works use labels as supplementary to construct prototypes of support videos, they can not use this information for query videos. The labels are not used efficiently. (b) Most of the works ignore the motion feature of video, although the motion features are essential for distinguishing. We proposed a Consistency Prototype and Motion Compensation Network(CLIP-CP$M^2$C) to address these issues. Firstly, we use the CLIP for multi-modal few-shot action recognition with the text-image comparison for domain adaption. Secondly, in order to make the amount of information between the prototype and the query more similar, we propose a novel method to compensate for the text(prompt) information of query videos when text(prompt) does not exist, which depends on a Consistency Loss. Thirdly, we use the differential features of the adjacent frames in two directions as the motion features, which explicitly embeds the network with motion dynamics. We also apply the Consistency Loss to the motion features. Extensive experiments on standard benchmark datasets demonstrate that the proposed method can compete with state-of-the-art results. Our code is available at the URL: https://github.com/xxx/xxx.git.

==> sec/4_experiments.tex <==
\section{Experiments}
\subsection{Datasets}
To evaluate our model, we design and conduct the experiments on five datasets which are used for few-shot action recognition, including Kinetics400\cite{carreira2017quo-kinetics}, SSv2-Full\cite{goyal2017something}, SSv2-small\cite{goyal2017something},  UCF101\cite{soomro2012ucf101} and HMDB51\cite{kuehne2011hmdb}. 
For SSv2-small and Kinesics, we use the split method of CMN\cite{zhu2018compound}, CMN-J\cite{zhu2020label}. The split method randomly selects a mini-dataset containing 100 classes, including 64 classes for training, 12 for validation, and 24 for testing, of which each class consists of 100 samples. 
For SSv2-Full, we follow the OTAM\cite{cao2020few-otam} split method. The difference between SSv2-Full and SSv2-small is the former uses all samples of a class. This method contains $77500/1926/2854$ videos for $train/val/test$ respectively.
The HMDB51 contains 31 classes for training, 10 classes for validation, and 10 classes for testing, with $4280/1194/1292$ videos for $train/val/test$.
For the UCF101, there are 70 classes for training, 10 classes for validation, and 21 classes for testing. It contains $9154/1421/2745$ videos for $train/val/test$ respectively. 
The split methods of HMDB51 and UCF101 follow ARN\cite{zhang2020few-ARN}.



\subsection{Implementation Details}
We follow the previous work TSN \cite{wang2016temporal-tsn} for the video frame. 8 frames are sparsely and uniformly sampled from each video. During training, we flip each frame horizontally and randomly crop the center region of 224 × 224 for data augmentation. For the Vision Language Model-CLIP, we use both the version encoder with ResNet50 and VIT-B/16. The optimizer we selected is Adam \cite{2014Adam}, and the learning rate is 0.00001. For training, we thus average gradients and backpropagate once every 16 iterations. For testing, we use only the center crop to augment the video. For inference, there are 10,000 episodes, and the average accuracy of this episode is reported in our experiment. We use the OTAM \cite{cao2020few-otam} as comparison methods for the experiments.


\subsection{Comparison with previous works}
We compare our model with the state-of-the-art methods, and our baseline is the CLIP-FSAR.

\begin{table*}[htbp]
  \centering
  \caption{Comparison on UCF101 and HMDB51. Accuracies for 5-way, 3-shot, and 1-shot settings are shown. $\diamond$ means our implementation
  }
  \vspace{-0.4em}
  \textbf{}
    \label{table:1}
    \scalebox{0.66}{
    \begin{tabular}{l|l|c|l|ccc|ccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[2]{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Modal Type}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Reference}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Backbone}} & \multicolumn{3}{c|}{HMDB51} & \multicolumn{3}{c}{UCF101} \\
          &       &       &       & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{3-shot} & \multicolumn{1}{c|}{5-shot} & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{3-shot} & \multicolumn{1}{c}{5-shot} \\
    \midrule
    ProtoNet \cite{snell2017prototypical_few_shot_learning2}& mono-modal&NeurIPS’2017&ResNet-50& 54.2&- &   68.4& 70.4& - &89.6 \\
    OTAM\cite{cao2020few-otam}  &mono-modal&CVPR’2020&ResNet-50&54.5 & - &66.1&79.9&- &88.9\\
    TRX \cite{perrett2021temporal-trx} &mono-modal&CVPR’2021&ResNet-50& $52.9^{\diamond}$ &- &75.6 &$77.3^{\diamond}$&-&96.1 \\
    STRM \cite{thatipelli2022spatio-strm}&mono-modal &CVPR’2022&ResNet-50& $54.1^{\diamond}$ &- &77.3&$79.2^{\diamond}$& - &96.9  \\
    HyRSM\cite{wang2022-hybrid}&mono-modal &CVPR’2022&ResNet-50&60.3  &71.7 & 76.0 & 83.9 & 93.0 & 94.7 \\
    MTFAN\cite{wu2022motion}&mono-modal&CVPR’2022&ResNet-50& 59.0 &- & 74.6 &84.8 & -& 95.1 \\
    TA2N\cite{li2022ta2n}&mono-modal&AAAI’2022&ResNet-50& 59.7 & - &73.9 &81.9  & -&95.1  \\
    HCL\cite{zheng2022few-hcl}&mono-modal&ECCV’2022&ResNet-50& 59.1 & - &76.3 &82.6  & -&94.5  \\
    TADRNet\cite{2023Task-AwareDual-Representation}&mono-modal&TCSVT'2023&ResNet-50&64.3&74.5&78.2&86.7&94.3&96.4 \\
    MoLo\cite{wang2023molo} &mono-modal&CVPR'2023&ResNet-50& 60.8&72.0&77.4& 86.0&93.5&95.5  \\
    AMeFu-Net(2020)\cite{fu2020depth}&multi-modal&MM’2020&ResNet-50&60.2 &- &75.5& 85.1&-&95.5\\
    SRPN(2021)\cite{wang2021semantic}& multi-modal &MM'2021&ResNet-50 &61.6 & 72.5 &76.2 & 86.5 & 93.8  & 95.8   \\
    TAda-Net(2022)\cite{wang2022task}   & multi-modal& MMSP'2022&ResNet-50&60.8 & 71.8 &76.4  & 85.7 & 93.3 &95.7  \\
    AMFAR(2023)\cite{wanyan2023active}  & multi-modal&CVPR'2023&ResNet-50& 73.9 &- & 87.8& 91.2 &- & 99.0 \\
    CLIP-FSAR(2023)\cite{wang2023CLIP}& multi-modal&IJCV'2023&CLIP-RN50 &  69.4  & 78.3 & 80.7  &92.4 & 95.4 &97.0 \\ 
    CLIP-FSAR(2023)\cite{wang2023CLIP}& multi-modal&IJCV'2023&CLIP-VIT-B &  77.1  & 84.1 & 87.7  &97.0 & 98.5 & 99.1 \\  
    \midrule
\rowcolor{gray!15}    CLIP-CP$\mathrm{M^2}$C      &multi-modal&-&CLIP-RN50& 66.3 & 78.4 $\uparrow$  & 81.2$\uparrow$ & 91.1& 96.2$\uparrow$& 97.4$\uparrow$  \\
\rowcolor{gray!15}    CLIP-CP$\mathrm{M^2}$C      &multi-modal&-&CLIP-VIT-B& 75.9  & 84.4 $\uparrow$ & 88.0$\uparrow$ &  95.0 &  98.1     & 98.6  \\
    \bottomrule
    \end{tabular}%
    }
\end{table*}%

\textbf{Result of UCF101 and HMDB51.}
The standard 5-way 1-shot, 3-shot, and 5-shot settings are scheduled in the experiment.
\cref{table:1} shows the comparison with various state-of-the-art methods. 
\textbf{HMDB51}:
Compared with CLIP-FSAR(RN50), our CLIP-CP$\mathrm{M^2}$C(RN50) brings
$0.5\% (80.7\% \rightarrow 81.2\%)$, 
$0.1\% (78.3\% \rightarrow  78.4\%)$ improvements under the 5-shot and 3-shot settings. 
Compared with CLIP-FSAR(VIT), our CLIP-CP$\mathrm{M^2}$C(VIT) brings
$0.3\% (87.7\% \rightarrow  88.0\%)$, 
$0.3\% (84.1\% \rightarrow 84.4\%)$ improvements under the 5-shot and 3-shot settings. 
\textbf{UCF101}: 
compared with CLIP-FSAR(RN50), our CLIP-CP$\mathrm{M^2}$C(RN50) brings
$0.4\% (97.0\% \rightarrow  97.4\%)$, 
$0.8\% (95.4\% \rightarrow  96.2\%)$ gains under the 5-shot and 3-shot settings.


\textbf{Results of Kinetics and SSv2.}
\cref{table:2} shows the comparison with various methods. 
\textbf{Kinetics}:
compared with CLIP-FSAR(RN50), our CLIP-CP$\mathrm{M^2}$C(RN50) brings 
$0.7\% (90.8\% \rightarrow 91.5\%)$,
$1.1\% (92.0\% \rightarrow 93.1\%)$ 
performance improvements for the 3-shot and 5-shot.
We can see under the 3-shot and 5-shot settings, CLIP-FSAR(RN50) can achieve the highest accuracy among the RN50-based methods.
Except for the 1-shot settings, our CLIP-CP$\mathrm{M^2}$C(VIT) achieves the highest accuracy.
\textbf{SSv2-Full}:
compared with CLIP-FSAR(RN50), our CLIP-CP$\mathrm{M^2}$C(RN50) brings 
$1.1\% (60.7\% \rightarrow 61.8\%)$, 
$1.2\% (62.8\% \rightarrow 64.0\%)$ performance improvements for the 3-shot and 5-shot.
The accuracy of CLIP-CP$\mathrm{M^2}$C(VIT) under 3-shot and 5-shot is higher than CLIP-FSAR(VIT).
\textbf{SSv2-small}: 
The accuracy of CLIP-CP$\mathrm{M^2}$C(RN50) is 
$0.8\% (54.0\% \rightarrow 54.8\%)$ higher than the CLIP-FSAR(RN50) under the 3-shot, 
and $1.3\% (55.8\% \rightarrow 57.1\%)$ higher under 5-shot.
The accuracy is the highest among the RN50-based models.
The accuracy of CLIP-CP$\mathrm{M^2}$C(VIT) under 5-shot is higher than CLIP-FSAR(VIT) and the 3-shot accuracy is a little lower.

Except for the 1-shot setting, our CLIP-CP$\mathrm{M^2}$C is leading for other models and achieves \textbf{state-of-the-art} under the Kinetics, HMDB51, SSv2-small, and SSv2-Full. We can see that the accuracies of 1-shot are slightly lower than CLIP-FSAR. This reason may be due to the fact that under the 1-shot setting, the negative impact of noise caused by the introduction of the fake-labeled query is greater than the positive contribution of using the fake-labeled query to enhance the amount of information. But our 1-shot results are still higher than most of the methods. 

\begin{table*}[htbp]
  \centering
  \caption{Comparison on Kinetics and SSv2 datasets. Accuracy results for 5-way, 3-shot, and 1-shot settings are shown. $\diamond$ means the results of our implementation (the data in parentheses represents the published data).}
  \vspace{-0.4em}
    \label{table:2}
    \scalebox{0.66}{
    \begin{tabular}{l|l|c|l|ccc|ccc|ccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[2]{*}{Method}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Modal Type}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Reference}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Backbone}} & \multicolumn{3}{c|}{Kinetics} & \multicolumn{3}{c|}{SSv2-Full} & \multicolumn{3}{c}{SSv2-small} \\
          &       &       &       & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{3-shot} & \multicolumn{1}{c|}{5-shot} & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{3-shot} & \multicolumn{1}{c|}{5-shot} & \multicolumn{1}{c}{1-shot} & \multicolumn{1}{c}{3-shot} & \multicolumn{1}{c}{5-shot} \\
    \midrule
    ProtoNet \cite{snell2017prototypical_few_shot_learning2}& mono-modal&NeurIPS’2017&ResNet-50& 65.4 &-&77.9&-& &-&33.6 &- & 43.0 \\
    Matching Net\cite{vinyals2016matching—few_shot_learning5}&mono-modal&NeurIPS’2016 &ResNet-50 &53.3& -& 74.6 &-&-&-& 34.4 & -&43.8 \\
    OTAM\cite{cao2020few-otam}          &mono-modal&CVPR’2020&ResNet-50&73.0 &- &85.5 &42.8 &- & 52.3 &$38.9^{\diamond}$ &- & $48.1^{\diamond}$ \\
    TRX \cite{perrett2021temporal-trx}  &mono-modal&CVPR’2021&ResNet-50& $63.4^{\diamond}$(63.6)  &- & $85.1^{\diamond}$(85.9) &42.0 &-& $63.0^{\diamond}$(64.6)  &36.0 &-& $56.3^{\diamond}$(59.4) \\
    STRM \cite{thatipelli2022spatio-strm}&mono-modal &CVPR’2022&ResNet-50& $65.3^{\diamond}$ & -  &$85.9^{\diamond}$(86.7)  &$42.9^{\diamond}$ &- &$64.8^{\diamond}$(68.1) &  &- &   \\
    HyRSM\cite{wang2022-hybrid}         &mono-modal &CVPR’2022&ResNet-50& 73.7  &83.5 & 86.1 &54.3  & 65.1  &  69.0 & 40.6 & 52.3  &56.1  \\
    MTFAN\cite{wu2022motion}            &mono-modal&CVPR’2022&ResNet-50& 74.6  &- & 87.4 &45.7 &  -  &  60.4 & - & -  &-  \\
    TA2N\cite{li2022ta2n}               &mono-modal&AAAI’2022&ResNet-50&72.8& -& 85.8 & 47.6 & -&61.0  & - & - & -   \\
    HCL\cite{zheng2022few-hcl}               &mono-modal&AAAI’2022&ResNet-50&73.7& -& 85.8 & 47.3 & -&64.9  &38.7& - & 55.4   \\
    TADRNet\cite{2023Task-AwareDual-Representation}&mono-modal&TCSVT'2023&ResNet-50& 75.6 & 84.8 & 87.4  &43.0 &-  &61.1&- & - &- \\
    MoLo\cite{wang2023molo}             &mono-modal &CVPR'2023&ResNet-50&74.0 &83.7& 85.6 &56.6 &67.0& 70.6 & 42.7 &52.9& 56.4 \\
    AMeFu-Net(2020)\cite{fu2020depth}   &multi-modal&MM’2020&ResNet-50& 74.1  &- &86.8 &- &-&- & - &-& - \\
    CMN++(2020)\cite{zhu2020label}      &multi-modal &TRAMI'2020&ResNet-50&60.5 &75.6 &78.9 & 36.2& 44.6 & 44.8 & - &-  &-  \\
    SRPN(2021)\cite{wang2021semantic}   & multi-modal &MM'2021&ResNet-50&75.2 & 84.7 &87.1  & -   & -   & -   & -  &  -  & - \\
    AMFAR(2023)\cite{wanyan2023active}  & multi-modal&CVPR'2023&ResNet-50&80.1 & -& 92.6 &61.7& -& 79.5 & -  & -  &-   \\
    CLIP-FSAR(2023)\cite{wang2023CLIP}  & multi-modal&IJCV'2023&CLIP-RN50 &90.1&90.8&92.0& 58.7&60.7&62.8 & 52.1 &54.0&55.8\\ 
    CLIP-FSAR(2023)\cite{wang2023CLIP}  & multi-modal&IJCV'2023&CLIP-VIT-B &94.8&95.0&95.4& 62.1&68.3&72.1 & 54.6 &59.4&61.8\\ 
    \midrule
    \rowcolor{gray!15}    CLIP-CP$\mathrm{M^2}$C        &multi-modal&-&CLIP-RN50& 88.6 & 91.5 $\uparrow$ & 93.1$\uparrow$ & 58.0 & 61.8 $\uparrow$ & 64.0 $\uparrow$&   51.5 & 54.8 $\uparrow$ & 57.1 $\uparrow$  \\
    \rowcolor{gray!15}    CLIP-CP$\mathrm{M^2}$C        &multi-modal&-&CLIP-VIT-B&91.0 & 95.1 $\uparrow$ & 95.5 $\uparrow$ & 60.1 &  68.9 $\uparrow$ & 72.8 $\uparrow$ & 52.3 &  58.9 &  62.6 $\uparrow$ \\
    \bottomrule
    \end{tabular}%
    }
\end{table*}%


\subsection{Ablation Study}
\textbf{Analysis of Model Components.}
To validate the contributions of each module in our work, we give the experiment under 5-way, 5-shot settings on Kinetics, SSv2-Small, and HMDB51 datasets. The CLIP-RN50 is chosen as the backbone for the visual encoder. As shown in \cref{table:3}, it can be seen that by using CPM with Consistency Loss and also using the normal frame features and the motion features from the MC module, we can get the highest accuracy. For the Kinetics, it brings the accuracy of $93.1\%$. Also, Under the SSv2-Small, it gets $57.1\%$ with all the settings.  
Through the \cref{table:3}, 
we can conclude that 
(1) Consistency Loss can improve the recognition accuracy.
(2) The accuracy is higher using both normal frame features and motion features simultaneously than only using a single type.
(3) Motion feature features can supplement normal features to a certain extent.
(4) The recognition using motion features alone is workable, and the accuracies are acceptable.

\begin{table*}[htbp]
  \centering
  \caption{Ablation for the Analysis of Model Components. It is for CPM(Consistency Loss) and the Feature type we choose.}
  \vspace{-0.4em}
  \label{table:3}
   \scalebox{0.66}{
    \begin{tabular}{c|c|cc|c|c|c}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[2]{*}{serial No}} & \multicolumn{1}{c|}{CPM} & \multicolumn{2}{c|}{Feature Type} & Kinetics & SSv2-Small & \multicolumn{1}{l}{HMDB51} \\
          & \multicolumn{1}{c|}{(Consistency-loss)} & Normal & Motion & 5-shot & 5-shot & \multicolumn{1}{l}{5-shot} \\
    \midrule
      (1)    & \ding{51}  & \ding{51}& \ding{51}  &93.1  & 57.1 & 81.2 \\
      (2)    & \ding{51}  & \ding{51}& \ding{55}  &92.8  & 55.8 & 81.0 \\
      (3)    & \ding{51}  & \ding{55}& \ding{51}  &91.6  & 56.4 & 80.5 \\
      (4)    & \ding{55}  & \ding{51}& \ding{51}  &92.6  & 56.4 & 80.8 \\
      (5)    & \ding{55}  & \ding{51}& \ding{55}  &92.3  & 55.4 & 80.1 \\
      (6)    & \ding{55}  & \ding{55}& \ding{51}  &90.9  & 55.9 & 79.9 \\
    \bottomrule
    \end{tabular}%
    }
\end{table*}%

\textbf{Analysis of Domain Adaption.}
To check the affection of the Domain Adaption, we use Kinetics and SSv2-Small under 1-shot and 5-shot settings with Consistency Loss for normal and motion features. In \cref{table:4}, the accuracy with Domain Adaption is higher than without it. It indicates that Domain Adaption, similar to many previous CLIP-related works, does contribute to our model.
\begin{table}[htbp]
  \centering
  \caption{Ablation for Domain Adaption in our model.}
  \vspace{-0.4em}
  \label{table:4}
  \scalebox{0.66}{
    \begin{tabular}{c|cc|cc}
    \toprule
    \multirow{2}[2]{*}{Domain-Adaption} & \multicolumn{2}{c|}{Kinetics} & \multicolumn{2}{c}{SSv2-Small} \\
          & 1-shot & 5-shot & 1-shot  & 5-shot \\
    \midrule
      \ding{51} &88.6&93.1& 51.5& 57.1 \\
      \ding{55} &87.3&92.4& 51.0  & 56.0 \\
    \bottomrule
    \end{tabular}%
    }
\end{table}%


\begin{figure}
\setlength{\belowcaptionskip}{-0.5cm} %调整图片标题与下文距离
\centering
\includegraphics[width=6.6cm]{hyper-motion.pdf}
\caption{\label{fig:parameter}The sensitivity of the hyper-parameter $\alpha$.
} 
\label{fig:3}
\end{figure}

\textbf{Hyper-parameter sensitivity of Motion analysis.}
In our work, a hyper-parameter balances the contribution of motion level and normal frame level distance. In \cref{fig:3}, we can observe that the parameter has an impact on the performance. According to \cref{fig:3}, in the experiments, we keep the hyper-parameter to be $1$.

The supplementary shows the model's visualization. 
